DSAF: A Dual-Stage Adaptive Framework for Numerical Weather Prediction Downscaling

While widely recognized as one of the most substantial weather forecasting methodologies, Numerical Weather Prediction (NWP) usually suffers from relatively coarse resolution and inevitable bias due to tempo-spatial discretization, physical parametrization process, and computation limitation. With the roaring growth of deep learning-based techniques, we propose the Dual-Stage Adaptive Framework (DSAF), a novel framework to address regional NWP downscaling and bias correction tasks. DSAF uniquely incorporates adaptive elements in its design to ensure a flexible response to evolving weather conditions. Specifically, NWP downscaling and correction are well-decoupled in the framework and can be applied independently, which strategically guides the optimization trajectory of the model. Utilizing a multi-task learning mechanism and an uncertainty-weighted loss function, DSAF facilitates balanced training across various weather factors. Additionally, our specifically designed attention-centric learnable module effectively integrates geographic information, proficiently managing complex interrelationships. Experimental validation on the ECMWF operational forecast (HRES) and reanalysis (ERA5) archive demonstrates DSAF's superior performance over existing state-of-the-art models and shows substantial improvements when existing models are augmented using our proposed modules. Code is publicly available at https://github.com/pengwei07/DSAF.

==> loss_function.tex <==
\subsection{Loss Function. }
In our study, we tackle the complexities of diverse weather factors through a two-stage approach: correction and downscaling, similar to a multi-task learning setup. Balancing the loss terms of each weather factor is crucial, given their distinct characteristics within the data. With the DSAF, we merge the losses from both stages, resulting in a dual-task loss function. We also incorporate physical constraints linking wind speed and pressure weather conditions. The total loss function, $\mathrm{loss}_{\mathrm{DSAF}}$, is optimized to determine the best parameters $\theta$:
\begin{equation}
\vspace{-1mm}
\left\{
\begin{aligned}
& \mathrm{loss}_{\mathrm{DSAF}} = \mathrm{loss}_0 + \mathrm{loss}_1 + \lambda_{\text{reg}}\mathrm{loss}_{\text{reg}},\\
&\mathrm{loss}_{0} = \mathrm{MSE}(\mathbf{Y}_L, \mathbf{Y}_L^{*}),\\
&\mathrm{loss}_{1} = \mathrm{MSE}(\mathbf{Y}, \mathbf{Y}^{*}),
\end{aligned}
\right.
\end{equation}
where $\mathbf{Y}_L^{*}$ is the low-resolution observed data derived from real high-resolution data, $\mathbf{Y}^{*}$. The terms $\mathrm{loss}_{0}$ and $\mathrm{loss}_{1}$ represent correction and downscaling losses. Moreover, $\mathrm{loss}_{\text{reg}}$ is the spatial-physical constraint between wind speed ($\mathbf{u}$) and surface pressure ($\mathbf{p}$), following the generalized Poisson equation. The coefficient $\lambda_{\text{reg}}$ adjusts this loss constraint's weight.\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Integrating Uncertainty.} Adapting from \cite{kendall2018multi}, we employ the uncertainty weighing approach given the dual nature of weather factor correction and downscaling. For multiple distinct weather factors, the loss function is:
\begin{equation}
\vspace{-1mm}
\begin{aligned}
& \mathrm{loss}_i(\theta)= \sum_{j=1}^{M} \lambda_j^i L_j^i(\theta) = \sum_{j=1}^{M} \lambda_j^i \mathrm{MSE}(\mathbf{Y}_j^i, \hat{\mathbf{Y}}_j^i), i=0,1,
\end{aligned}
\vspace{-1mm}
\end{equation}
where $\lambda_j^i$ is the optimized loss hyperparameter. The terms represent channels of low-resolution input and its ground truth and high-resolution output with its corresponding truth, shedding light on individual weather factor behavior across resolutions.\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Spatial-physical Constraint.} The dynamic relationship between wind speed and pressure is an important meteorological research topic. Basically, as the pressure gradient intensifies, it often precipitates a surge in wind speed \cite{walker1990effects, kwak2007analysis}. This foundational relation can be represented by the general Poisson equation:
\begin{equation}
Loss_{reg} = \nabla^2 p + \nabla \cdot (\mathbf{u} \cdot \nabla \mathbf{u}). 
\end{equation}
To further emphasize, in our practical observations, pressure's downscaling emerges as more intuitive compared to other meteorological variables. Such insights prompted us to harness pressure for the refined correction of wind speed. Driving the $Loss_{reg}$ towards zero accentuates the modeling of this relationship. Central to this endeavor is our strategic incorporation of the Element-wise Product (EWP). This tool serves as a linchpin, approximating the gradient operator $\nabla$ with heightened precision. By employing the expressions $\prod_{j=0}^{3} (k_{j} \circledast p + b_j)$ and $\prod_{j=0}^{4} (k_{j} \circledast p + b_j)$, we can, respectively, mirror the dynamics of $\nabla^2 p$ and $\nabla \cdot (\mathbf{u} \cdot \nabla \mathbf{u})$. Furthermore, leveraging Conv $1\times1$, we extract the terms $k_{j} \circledast p + b_j$, with specific attention to the order nuances when $j=3$ and $j=4$.

==> table1_1.tex <==
% 表1:和baseline模型的对比
\begin{table*}[h]
\centering
\footnotesize
\caption{\footnotesize Downscaling performance comparison at each weather factor on the ECMWF operational forecast (HRES) and reanalysis (ERA5) with RMSE for the 2x scale. \textbf{Bold} and \underline{Underline} indicate the best and second best performance, respectively. $\Delta$ denotes the relative improvement between DSAF and baselines/Bicubic.}
\label{tab1_1}
%\vspace{-1mm}
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
Channel & sp & 2t & d2m & skt & 10u & 10v & 100u & 100v \\
\midrule
Scale      & 2x & 2x & 2x & 2x & 2x & 2x & 2x & 2x\\
\midrule
Bicubic    
&0.82&1.71&1.99&1.61&1.21&1.28&1.68&1.78 \\
FSRCNN 
&0.43 &1.20 &1.24 &1.29 &1.09 &1.07 &1.19 &1.23\\
ResDeepD 
&0.30 &1.18 &1.26 &1.20 &1.00 &0.97 &1.09 &1.08\\
EDSR     
& 0.46 & 1.21 & 1.30  & 1.24 & 1.02 & 1.00 & 1.14 & 1.17 \\
C\_EDSR     
& 0.22 & 1.19 & 1.26 & 1.12 & \underline{0.75} & 0.78 & 1.02 & 1.07 \\
RCAN       
& 0.57 & 1.22 & 1.29 & 1.28 & 1.03 & 1.00 & 1.16& 1.19  \\
C\_RCAN     
& \underline{0.20} & \underline{1.00} & \underline{1.13} & \underline{0.99} & 0.81 & \underline{0.76} & \underline{1.002} 
& \underline{0.98} \\ 
GINE
&  &  &  &  &  &  &  &   \\
SRGAN
&  &  &  &  &  &  &  &   \\
D\_C\_DSAF &0.21 &1.01 &1.15 &1.02 &0.78 &0.77 &1.01&1.03\\
DSAF (ours) &\textbf{0.18} & \textbf{0.96} & \textbf{1.03} & \textbf{0.90} & \textbf{0.73} & \textbf{0.75}& \textbf{1.001} &\textbf{0.94}\\
\midrule
$\Delta$ Best  
& 10.00\% 
& 4.00\% 
& 8.85\% 
& 9.09\% 
& 2.67\% 
& 1.32\% 
& 0.20\%  
& 4.08\% \\
%\hline
$\Delta$ Bicubic 
& 78.05\% 
& 43.86\% 
& 48.24\% 
& 44.10\% 
& 39.67\% 
& 41.41\% 
& 40.48\%
& 47.19\%\\
\toprule
\end{tabular}
%\vspace{-1mm}
\end{table*}

==> table1_2.tex <==
% 表1:和baseline模型的对比
\begin{table*}[h]
\centering
\footnotesize
\caption{\footnotesize Downscaling performance comparison at each weather factor on the ECMWF operational forecast (HRES) and reanalysis (ERA5) with RMSE for the 4x scale. \textbf{Bold} and \underline{Underline} indicate the best and second best performance, respectively. $\Delta$ denotes the relative improvement between DSAF and baselines/Bicubic.}
\label{tab1_2}
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
Channel & sp & 2t & d2m & skt & 10u & 10v & 100u & 100v \\
\midrule
Scale      & 4x & 4x & 4x & 4x & 4x & 4x & 4x & 4x\\
\midrule
Bicubic    
&1.22&1.84&2.06&1.85&1.27&1.36&1.76&1.87 \\
FSRCNN 
&0.56&1.23&1.39&1.33&1.12&1.09&1.20&1.27\\
ResDeepD 
&0.32&1.20&1.29&1.23&1.07&1.01&1.11&1.11\\
EDSR     
&0.55&1.27& 1.38& 1.39& 1.11& 1.11& 1.21& 1.22 \\
C\_EDSR     
& 0.18& 1.11& 1.20& 1.10& 0.74& \underline{0.73} & 1.04& 0.98 \\
RCAN       
& 0.61 & 1.26& 1.38 & 1.31 & 1.10 & 1.10 & 1.19& 1.20  \\
C\_RCAN     
& \underline{0.190}& \underline{0.99}& \underline{1.09}  & \underline{0.98} & \underline{0.728}  & 0.74  & \underline{1.00} & \underline{0.95} \\ 
GINE
&  &  &  &  &  &  &  &   \\
SRGAN
&  &  &  &  &  &  &  &   \\
D\_C\_DSAF 
&0.191 &1.00 &1.10 &1.01 &0.73 &0.76 &1.02 &1.01\\
DSAF (ours)
& \textbf{0.16}  & \textbf{0.96} & \textbf{1.01} & \textbf{0.88} & \textbf{0.721} & \textbf{0.72} & \textbf{0.99} & \textbf{0.92} \\
\midrule
$\Delta$ Best  
& 10.00\% 
& 4.00\% 
& 8.85\% 
& 9.09\% 
& 2.67\% 
& 1.32\% 
& 0.20\%
& 4.08\% \\
%\hline
$\Delta$ Bicubic 
& 78.05\% 
& 43.86\% 
& 48.24\%
& 44.10\% 
& 39.67\% 
& 41.41\% 
& 40.48\%
& 47.19\%\\
\toprule
\end{tabular}
%\vspace{-1mm}
\end{table*}

==> table1_all.tex <==
\begin{table*}[h]
    \centering
    \scriptsize
    %\tiny

    % 第一个表格
    \begin{minipage}{0.45\linewidth}
        \setlength{\tabcolsep}{2pt}
        \centering
        \caption{\footnotesize Downscaling performance comparison at each weather factor on the ECMWF operational forecast (HRES) and reanalysis (ERA5) with RMSE for the 2x scale. \textbf{Bold} and \underline{Underline} indicate the best and second best performance, respectively. $\Delta$ denotes the relative improvement between DSAF and baselines/Bicubic.}
        \label{tab1_1}
        \begin{tabular}{l|c|c|c|c|c|c|c|c}
        \toprule
        Channel & sp & 2t & d2m & skt & 10u & 10v & 100u & 100v \\
        %\midrule
        %Scale      & 2x & 2x & 2x & 2x & 2x & 2x & 2x & 2x\\
        \midrule
        Bicubic    
        &0.82&1.71&1.99&1.61&1.21&1.28&1.68&1.78 \\
        FSRCNN 
        &0.43 &1.20 &1.24 &1.29 &1.09 &1.07 &1.19 &1.23\\
        ResDeepD 
        &0.30 &1.18 &1.26 &1.20 &1.00 &0.97 &1.09 &1.08\\
        EDSR     
        & 0.46 & 1.21 & 1.30  & 1.24 & 1.02 & 1.00 & 1.14 & 1.17 \\
        C\_EDSR     
        & 0.22 & 1.19 & 1.26 & 1.12 & \underline{0.75} & 0.78 & 1.02 & 1.07 \\
        RCAN       
        & 0.57 & 1.22 & 1.29 & 1.28 & 1.03 & 1.00 & 1.16& 1.19  \\
        C\_RCAN     
        & \underline{0.20} & \underline{1.00} & \underline{1.13} & \underline{0.99} & 0.81 & \underline{0.76} & \underline{1.002} 
        & \underline{0.98} \\ 
        GINE
        &  &  &  &  &  &  &  &   \\
        SRGAN
        &  &  &  &  &  &  &  &   \\
        D\_C\_DSAF &0.21 &1.01 &1.15 &1.02 &0.78 &0.77 &1.01&1.03\\
        \textbf{DSAF} &\textbf{0.18} & \textbf{0.96} & \textbf{1.03} & \textbf{0.90} & \textbf{0.73} & \textbf{0.75}& \textbf{1.001} &\textbf{0.94}\\
        \midrule
        $\Delta$ Best  
        & 10.0\% 
        & 4.0\% 
        & 8.9\% 
        & 9.1\% 
        & 2.7\% 
        & 1.3\% 
        & 0.2\%  
        & 4.1\% \\
        %\hline
        %$\Delta$ Bicubic 
        %& 78.1\% 
        %& 43.9\% 
        %& 48.2\% 
        %& 44.1\% 
        %& 39.7\% 
        %& 41.4\% 
        %& 40.5\%
        %& 47.2\%\\
        \toprule
        \end{tabular}
    \end{minipage}%
    % 这里的 '%' 符号确保没有额外的空间在两个 minipages 之间
    \hfill % 增加间距

    % 第二个表格
    \begin{minipage}{0.45\linewidth}
        \setlength{\tabcolsep}{2pt}
        \centering
        \caption{\footnotesize Downscaling performance comparison at each weather factor on the ECMWF operational forecast (HRES) and reanalysis (ERA5) with RMSE for the 4x scale. \textbf{Bold} and \underline{Underline} indicate the best and second best performance, respectively. $\Delta$ denotes the relative improvement between DSAF and baselines/Bicubic.}
        \label{tab1_2}
        \begin{tabular}{l|c|c|c|c|c|c|c|c}
        \toprule
        Channel & sp & 2t & d2m & skt & 10u & 10v & 100u & 100v \\
        %\midrule
        %Scale      & 4x & 4x & 4x & 4x & 4x & 4x & 4x & 4x\\
        \midrule
        Bicubic    
        &1.22&1.84&2.06&1.85&1.27&1.36&1.76&1.87 \\
        FSRCNN 
        &0.56&1.23&1.39&1.33&1.12&1.09&1.20&1.27\\
        ResDeepD 
        &0.32&1.20&1.29&1.23&1.07&1.01&1.11&1.11\\
        EDSR     
        &0.55&1.27& 1.38& 1.39& 1.11& 1.11& 1.21& 1.22 \\
        C\_EDSR     
        & 0.18& 1.11& 1.20& 1.10& 0.74& \underline{0.73} & 1.04& 0.98 \\
        RCAN       
        & 0.61 & 1.26& 1.38 & 1.31 & 1.10 & 1.10 & 1.19& 1.20  \\
        C\_RCAN     
        & \underline{0.190}& \underline{0.99}& \underline{1.09}  & \underline{0.98} & \underline{0.728}  & 0.74  & \underline{1.00} & \underline{0.95} \\ 
        GINE
        &  &  &  &  &  &  &  &   \\
        SRGAN
        &  &  &  &  &  &  &  &   \\
        D\_C\_DSAF 
        &0.191 &1.00 &1.10 &1.01 &0.73 &0.76 &1.02 &1.01\\
        \textbf{DSAF}
        & \textbf{0.16}  & \textbf{0.96} & \textbf{1.01} & \textbf{0.88} & \textbf{0.721} & \textbf{0.72} & \textbf{0.99} & \textbf{0.92} \\
        \midrule
        $\Delta$ Best  
        & 10.0\% 
        & 4.0\% 
        & 8.9\% 
        & 9.1\% 
        & 2.7\% 
        & 1.3\% 
        & 0.2\%
        & 4.1\% \\
        %\hline
        %$\Delta$ Bicubic 
        %& 78.05\% 
        %& 43.86\% 
        %& 48.24\%
        %& 44.10\% 
        %& 39.67\% 
        %& 41.41\% 
        %& 40.48\%
        %& 47.19\%\\
        \toprule
        \end{tabular}
    \end{minipage}

\end{table*}


==> table2_1.tex <==
% 表2转换为表1的格式
\begin{table}[h]
\setlength{\tabcolsep}{3pt}
\centering
\caption{Comparison of different ways of Multi-task learning and Ablation study for the 2x scale.}
\label{tab2_1}
%\scriptsize
\footnotesize
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
Channel & sp & 2t & d2m & skt & 10u & 10v & 100u & 100v \\
%\midrule
%Scale      & 2x & 2x & 2x & 2x & 2x & 2x & 2x & 2x\\
\midrule
Base\_DSAF     
&0.82&1.71&1.99&1.61&1.21&1.28&1.67&1.78\\
DeConv\_DSAF 
&0.41&1.29&1.30&1.11&0.82&0.99&1.07&1.14 \\
no\_TCA         
&0.41&1.23&1.26&1.10&0.79&0.89&1.02&1.00 \\\midrule
single       
&0.37&1.18&1.24&1.09&0.79&0.91&1.05&1.09 \\\midrule
Average      
&0.41&1.17&1.22&1.15&0.87&0.89&1.11&1.13\\
Adaptive     
&0.38&1.14&1.20&1.09&0.76&0.78&1.05&1.09\\\midrule
DSAF (ours)   
&\textbf{0.18}&\textbf{0.96}&\textbf{1.03}&\textbf{0.90}&\textbf{0.73}&\textbf{0.75}&\textbf{1.00}&\textbf{0.94} \\
\toprule
\end{tabular}
%\vspace{-2mm}
\end{table}

==> table2_2.tex <==
% 表2转换为表1的格式
\begin{table}[h]
\centering
%\footnotesize
\scriptsize
\caption{Comparison of different ways of Multi-task learning and Ablation study for the 4x scale.}
\label{tab2_2}
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
Channel & sp & 2t & d2m & skt & 10u & 10v & 100u & 100v \\
%\midrule
%Scale      & 4x & 4x & 4x & 4x & 4x & 4x & 4x & 4x\\
\midrule
Base\_DSAF     
&1.22&1.84&2.06&1.85&1.27&1.36&1.76&1.87 \\
DeConv\_DSAF 
&0.40&1.09&1.16&1.00&0.84&0.83&1.14&1.13 \\
no\_TCA         
&0.39&1.08&1.16&1.01&0.76&0.84&1.06&1.00 \\\midrule
single       
&0.33&1.08&1.15&1.00&0.76&0.79&1.10&1.05 \\\midrule
Average      
&0.36&1.12&1.18&1.08&0.83&0.85&1.10&1.17 \\
Adaptive     
&0.36&1.10&1.17&1.01&0.75&0.83&1.06&1.22 \\\midrule
DSAF (ours)   
&\textbf{0.16}&\textbf{0.96}&\textbf{1.01}&\textbf{0.88}&\textbf{0.72}&\textbf{0.72}&\textbf{0.99}&\textbf{0.92} \\
\toprule
\end{tabular}
%\vspace{-2mm}
\end{table}
